A Thorough Examination on Zero-shot Dense Retrieval

Recent years have witnessed the significant advance in dense retrieval (DR) based on powerful pre-trained language models (PLM). DR models have achieved excellent performance in several benchmark datasets, while they are shown to be not as competitive as traditional sparse retrieval models (e.g., BM25) in a zero-shot retrieval setting. However, in the related literature, there still lacks a detailed and comprehensive study on zero-shot retrieval. In this paper, we present the first thorough examination of the zero-shot capability of DR models. We aim to identify the key factors and analyze how they affect zero-shot retrieval performance. In particular, we discuss the effect of several key factors related to source training set, analyze the potential bias from the target dataset, and review and compare existing zero-shot DR models. Our findings provide important evidence to better understand and develop zero-shot DR models.

==> Zero-shot Dense Retrieval/subfile/1_intro.tex <==
\section{Introduction}
\label{section:intro}
With the massive success of pre-trained language models~(PLM)~\cite{bert2019naacl, brown2020language}, dense retrieval~(DR) has been empowered to become an essential technique in first-stage retrieval.
Instead of using sparse term-based representations, DR learns low-dimensional query and document embeddings for semantic matching, which has been shown to be competitive with or even better than sparse retrievers (\eg BM25)~\cite{dpr2020}. 
% One line of DR studies is designing pre-training methods~\cite{lu2021less, ouguz2021domain}, which usually incorporates task-specific loss during the pre-training process~\cite{gao2021unsupervised, pair}. While another line is designing specific fine-tuning methods in different aspects, \eg negative sampling~\cite{negative2020google, rocketqa}, improving efficiency~\cite{zhan2021jointly}, and joint training~\cite{sachan2021end, rocketqav2}.


Unlike sparse retrievers, DR models typically require training on sufficient labeled data to achieve good performance in a specific domain.
However, there are always new domains (or scenarios) that need to be dealt with for an information retrieval system, where little in-domain labeled data is accessable.
Therefore, it is crucial to investigate the retrieval capabilities of DR models under the \emph{zero-shot} setting, where DR models trained on an existing domain (called \emph{source domain}) is directly applied to another domain (called \emph{target domain}) with no available training data on the target domain.
Considering the large discrepancy between different domains, the zero-shot capability directly affects the widespread deployment of DR models in real-world applications.


Recently, a number of studies have been conducted to analyze the zero-shot capability of DR models~\cite{thakur2021beir, chen2022out}, and report that DR models have poor zero-shot retrieval performance when compared with lexical models such as BM25. However, existing works primarily focus on zero-shot performance across a wide range of tasks, and lacks a comprehensive and in-depth analysis on the influence of different settings affected by various factors. Thus, the derived findings may not hold under some specific settings, which cannot ensure an accurate understanding of the zero-shot retrieval capacity. For example,  our empirical analysis has revealed that BM25 is not the absolute leader compared with DR models under the zero-shot setting, and different source training sets result in different zero-shot performances (Section~\ref{sec:initial-analysis}).
As a result, a thorough examination of the zero-shot capacity of DR models is necessary.

Considering these issues, this paper aims to provide an in-depth empirical analysis of the zero-shot capability of DR models.
Specifically, we would like to conduct a more detailed analysis by analyzing the effect of different factors on retrieval performance.
Since the DR models are trained on the source domain data (called \emph{source training set}), we focus on the analysis by examining three major aspects of the source training set, including query set, document set, and data scale. Besides, we also consider other possible factors such as query type distribution, vocabulary overlap between source and target sets, and the bias of the target dataset. Our analysis is particularly interested in answering 
the research questions of
% (a) What about the overall zero-shot capability of DR models? Is it really that bad compared to sparse retrievers?
what influence factors affect the zero-shot capabilities of DR models and how does each of the influence factors affect such capability?
By our empirical analysis, we find that:

$\bullet$ The training data from the source domain has important effect on the zero-shot capability of the trained DR model, either the query set or document set in it (Section~\ref{sec:query-effect} and Section \ref{sec:document-effect}).

$\bullet$ Vocabulary overlap and query type distribution are potential factors that affect the zero-shot performance (Section~\ref{sec:query-overlap} and Section \ref{sec:query-type}).

$\bullet$ Increasing the query scale of source data can improve both the in-domain and out-of-domain performance of the DR model (Section~\ref{sec:query-scale}). 

$\bullet$ Increasing the document scale of the source domain may result in performance decrease (Section~\ref{sec:document-scale}). 

$\bullet$ The lexical bias~(overlap coefficient of queries and annotated documents) of some target datasets is probably one of the reasons that the performance of sparse retriever seems to be more robust than the DR model on existing benchmarks (Section~\ref{sec:bias}).
% Overall, (i) the training data from the source domain has important effect on the zero-shot capability of the trained DR model, either the query set or document set in it (Section~\ref{sec:query-effect} and Section \ref{sec:document-effect}).
% Among them, (ii) vocabulary overlap and query type distribution are potential factors that affect the zero-shot performance (Section~\ref{sec:query-overlap} and Section \ref{sec:query-type}).
% (iii) Increasing the query scale of source data can improve both the in-domain and out-of-domain performance of the DR model (Section~\ref{sec:query-scale}). 
% % When the scale is small, the performance tends to be more sensitive to it.
% (iv) Increasing the document scale of the source domain may result in performance decrease (Section~\ref{sec:document-scale}). 
% In addition, (v) the lexical bias~(overlap coefficient of queries and annotated documents) of some target datasets is probably one of the reasons that the performance of sparse retriever seems to be more robust than the DR model on existing benchmarks (Section~\ref{sec:bias}).

Besides, we also systematically review the recent advances in zero-shot DR. We summarize and categorize the key techniques that can improve the zero-shot performance (with an associated discussion of the potential influence factors). Our study provides an important work to understand and improve the zero-shot capacity of the DR model.



==> Zero-shot Dense Retrieval/subfile/2_preliminaries.tex <==
\section{Background and Setup}
In this section, we introduce the necessary background in this paper.

\subsection{Zero-shot Dense Retrieval}

We study the task of finding relevant documents with respect to a query from a large document set\footnote{Note that in this paper, ``document'' is a generalized concept that can be in a variety of text forms, such as passage, sentence, and article.}. In particular, we focus on \emph{dense retrieval}~(DR) approaches that learn low-dimensional semantic embeddings for both queries and documents and then measure the embedding similarities as the relevance scores. To implement DR approach, a PLM-based dual-encoder has been widely adopted~\cite{zhao2022dense, dpr2020, ANCE} by learning two separate text encoders for relevance matching. Compared with sparse retrieval models (\eg BM25), DR models highly rely on large-scale high-quality training data to achieve good performance~\cite{rocketqa, negative2020google}. 

We mainly consider the setting of zero-shot DR~\cite{thakur2021beir}, where the labeled data from \emph{target domain} is only available for testing. Besides, we assume that the labeled data from a different domain (called \emph{source domain}) can be used to train the DR models. Such a setting is slightly different from general zero-shot learning, where no labeled data is available at all. %As reported in \cite{thakur2021beir}, DR models seem to have a weak zero-shot retrieval capacity (trained on  source domain data only). 
This paper aims to present a deep and comprehensive analysis on the zero-shot capacity of DR models.  



\begin{table}[t]
    \scriptsize
    \renewcommand\tabcolsep{1.pt}
    \centering
    \begin{tabular}{lccccc}
        \toprule
        \textbf{Datasets} & \textbf{\#Train Q} & \textbf{\#Eval. Q} & \textbf{\#D} & \textbf{Q Len.} & \textbf{D Len.}\\
        \midrule
        Natural Questions~(NQ) & 58,812 & 3,610 & 21,015,324 & 9.2 & 100.0 \\
        MSMARCO~(MM) & 502,939 & 6,980 & 8,841,823 & 6.0 & 56.9 \\
        MSMARCOv2~(MMv2) & 277,144 & 8,184 & 138,364,198 & 5.9 & 47.5 \\
        HotpotQA~(HQA) & 72,928 & 5,901 & 21,015,324 & 20.0 & 100.0\\
        TriviaQA~(TQA) & 61,688 & 7,785 & 21,015,324 & 13.7 & 100.0 \\
        SearchQA~(SQA) & 117,384 & 16,980 & 21,015,324 & 14.6 & 100.0 \\ 
        NQ$_\text{MRQA}$ & 104,071 & 6,775 & 21,015,324 & 11.1 & 100.0 \\ 
        \midrule
        FiQA-2018 & 5,500 & 648 & 57,638 & 10.8 & 132.3\\
        SciFact & 809 & 300 & 5,183 & 12.4 & 213.6\\
        SciDocs & - & 1,000 & 25,637 & 9.4 & 176.2 \\
        BioASQ & 3,742 & 500 & 14,914,602 & 8.1 & 202.6 \\
        Quora & - & 10,000 & 522,931 & 9.5 & 11.4\\
        ArguAna & - & 1,406 & 8,674 & 193.0 & 166.8 \\
        \bottomrule
    \end{tabular}
    \caption{Dataset statistics, where ``Q'' denotes query and ``D'' denotes document. The upper part lists source datasets and the lower part lists target datasets in our zero-shot experiments. }
    \label{tab:dataset}
\end{table}


\subsection{Experimental Setup}
In this part, we set up our analysis experiments for zero-shot retrieval. 

\paratitle{Datasets}
\label{sec:dataset}
In order to comprehensively study the zero-shot capability of the DR model, we collect 12 popular datasets that cover multiple domains with different data characteristics. 
The statistics of the datasets is shown in Table~\ref{tab:dataset}. In Table~\ref{tab:dataset}, the upper part includes source datasets and the lower part includes target datasets.
In our experiment design, we select datasets that allow us to conduct controlled  experiments.
The target datasets are the representative datasets with multiple domains from BEIR~\cite{thakur2021beir} benchmark, that consists of multiple datasets for evaluating zero-shot performance of retrieval models. 
The detailed description of the datasets can be found in Appendix~\ref{app:dataset}.


\paratitle{Training Data Construction}  To examine the effect of query set and document set, which are two factors in source dataset, we incorporate a combination form of \emph{<\underline{Query set}, \underline{Document set}>} to denote the resources of query set and document set, where they can come from different domains or datasets. For example, ``<NQ, MM>'' in Table~\ref{tab:target-transfer} denotes that queries in NQ are used to construct training data with documents in MSMARCO.

There are two types of annotation including long answer and short answer, where long answer denotes the whole relative document and short answer denotes the short span that directly answers the query.
When examining the effects of query set and document set in the source dataset, we change the query set or document set respectively. In such cases, we leverage the annotated short answers to relabel the relevant documents in a new combined source dataset. Taking ``<NQ, MM>'' in Table~\ref{tab:target-transfer} as an example, we use queries in NQ and select candidates containing short answers as positives from MSMARCO document set, negatives are sampled from candidates without short answers.

% to construct training data on MSMARCO document set.
% For datasets with annotated short answers~(\eg NQ), positive documents are the top-ranked candidates that contain short answers, and negative samples are randomly sampled from candidates without containing the corresponding answer.
% For example, since NQ has short answer annotations, we can use queries in NQ to construct training data on any document set, which is not possible on MSMARCO.


\paratitle{Evaluation Metrics}
We use MRR@10 and Recall@50 as evaluation metrics. MRR@10 calculates the averaged reciprocal of the rank of the first positive document for a set of queries. Recall@50 calculates a truncated recall value at position 50 of a retrieved list. For space constraints, we denote MRR@10 and Recall@50 by M@10 and R@50, respectively. 
% Due to space constraints, we let ``E1'' and ``E2''  denote MRR@10 and Recall@50 evaluated by retriever, and ``E3'' denote MRR@10 evaluated by re-ranker. 


\subsection{Initial Analysis on MSMARCO and NQ}
\label{sec:initial-analysis}
To gain a basic understanding of zero-shot retrieval capacities, we conduct  analysis experiments on two well-known public datasets, MSMARCO and NQ, considering both in-domain (\emph{training} and \emph{testing} on the same dataset) and out-of-domain settings (\emph{training} and \emph{testing} on two different datasets). 


\begin{table}[t]
    \centering
    \scriptsize
    \renewcommand\tabcolsep{4.8pt}
    \begin{tabular}{l|cc|cc}
        \toprule
        \textbf{Target~($\rightarrow$)} & \multicolumn{2}{c|}{\textbf{NQ}}  & \multicolumn{2}{c}{\textbf{MSMARCO}} \\
        \textbf{Models (with source dataset)~($\downarrow$)}    & \textbf{M@10} & \textbf{R@50} &  \textbf{M@10} & \textbf{R@50} \\
        \midrule
        BM25 & 31.3 & 69.7 & 18.7 & 59.2 \\
                \hline
        ANCE (MSMARCO) & 39.9 & 78.9 & 33.0 & 79.1 \\
        % ANCE (NQ) & 39.9 & 78.9 & 33.0 & 79.1 \\
               \hline
        RocketQAv2 (MSMARCO) & 50.8 & 83.2 & \textbf{38.8} & \textbf{86.5}  \\
        RocketQAv2 (NQ)  & \textbf{61.1} & \textbf{86.9} & 22.4 & 67.2  \\ 
        \bottomrule
    \end{tabular}
    \caption{Evaluation results of models trained on MSMARCO and NQ.}
    \label{tab:initial}
\end{table}

\paratitle{Backbone Selection} We select RocketQAv2~\cite{rocketqav2} as the major DR model for study, which is one of the state-of-the-art DR models. We train models on MSMARCO and NQ, and use RocketQAv2 (MSMARCO) and RocketQAv2 (NQ) denote RocketQAv2 model trained on MSMARCO and NQ, respectively.
For comparison, we adopt the ANCE~\cite{ANCE} and BM25 as two baselines, and report their corresponding performance. 
From Table~\ref{tab:initial}, we find that the performance of RocketQAv2 outperform ANCE evaluating on the two datasets (trained on MSMARCO). Thus, in the following experiments, we select RocketQAv2 as the backbone model. 

\paratitle{Results on NQ and MSMARCO}
In addition, it also can be observed in Table~\ref{tab:initial} that the two DR models are better than BM25 when evaluated on NQ and MSMARCO. 
Furthermore, The performance gap evaluating on MSMARCO development set between RocketQAv2 (NQ) and RocketQAv2 (MSMARCO)~(38.8 vs 22.4) is greater than the performance gap on NQ test set~(61.1 vs 50.8), indicating that the DR model trained on MSMARCO is stronger than that trained on NQ.


\paratitle{Results on Target Datasets} 
We also test the zero-shot performance of RocketQAv2 (trained on NQ and MSMARCO) on six target datasets, including SciDocs, SciFact, FiQA, BioASQ, Quora, and ArguAna. As shown in Table~\ref{tab:target-transfer}~(part $A$), RocketQAv2 (MSMARCO) outperforms RocketQAv2 (NQ) on most target datasets, showing that \textbf{the DR model trained on MSMARCO has a stronger zero-shot capability}.
Moreover, it can be observed that BM25 outperforms DR models significantly on SciFact and BioASQ, and is also competitive on other target datasets, which is a strong zero-shot retrieval baseline.


Through the initial experiments, we can see that models trained on the two source datasets have different zero-shot performance when tested on diverse target datasets. 
It is difficult to directly draw concise conclusions about the zero-shot capacities of DR models, given the significant performance variations in different settings. 
Considering this issue, in what follows, we systematically investigate \emph{what} factors are relevant and \emph{how} they affect the zero-shot performance in multiple aspects.

==> Zero-shot Dense Retrieval/subfile/3_analysis.tex <==


\section{Experimental Analysis and Findings}
\label{sec:analysis}
% Since DR models are trained on labeled relevance judgments from a source domain in the zero-shot setting, we speculate that 
% source training set has important effects on the zero-shot retrieval capacity. For this purpose, 
In this section, we conduct a detailed analysis about multiple factors of the source training set, including source query set, source document set, and data scale. Besides, we also analyze the effect of the bias from the target dataset. 


\begin{table*}[htbp!]
    \scriptsize
    \centering
    \renewcommand\tabcolsep{3.7pt}
    \begin{tabular}{l|cc|cc|cc|cc|cc|cc|cc}
        \toprule
        \textbf{Target~($\rightarrow$)} & \multicolumn{2}{c|}{\textbf{SciDocs}} & \multicolumn{2}{c|}{\textbf{SciFact}}  & \multicolumn{2}{c|}{\textbf{FiQA-2018}} & \multicolumn{2}{c|}{\textbf{BioASQ}} & \multicolumn{2}{c|}{\textbf{Quora}} & \multicolumn{2}{c|}{\textbf{ArguAna}} & \multicolumn{2}{c}{\textbf{Average}} \\
        \textbf{Source~($\downarrow$)} & \textbf{M@10} & \textbf{R@50} &  \textbf{M@10} & \textbf{R@50} & \textbf{M@10} & \textbf{R@50} & \textbf{M@10} & \textbf{R@50} & \textbf{M@10} & \textbf{R@50} & \textbf{M@10} & \textbf{R@50} & \textbf{M@10} & \textbf{R@50} \\
        \hline
        \multicolumn{3}{l}{\colorbox{gray!30}{$A$. Initial Experiment}} \\
        \midrule
        BM25 & 20.7 & 57.8 & \textbf{62.2} & \textbf{86.7} & 29.7 & 63.7 & \textbf{46.0} & \textbf{73.0} & 73.8 & 95.7 & 20.8 & \textbf{86.9} & \textbf{42.2} & \textbf{77.3}\\
        <NQ, Wikipedia> & \textbf{24.3} & 61.2 & 40.5 & 73.7 & 23.9 & 61.6 & 24.1 & 49.4 & \textbf{76.8} & \textbf{97.8} & 9.7 & 65.9 & 33.2 & 68.3 \\
        <MM, MM> & 24.1 & \textbf{63.7} & 48.0 & 77.0 & \textbf{35.1} & \textbf{71.3} & 30.9 & 55.0 & 71.4 & 97.6 & \textbf{21.6} & 85.8 & 38.5 & 75.1 \\
        % MSMARCO~(ANCE) & 22.7 & 22.2 & -& 48.3 & 75.6 & -& 36.3 & 51.6 & -& 42.8 & 43.0 & -& 84.5 & 97.9 & -& 33.6 & 89.7 & - &\\
        \hline\midrule
        \multicolumn{3}{l}{\colorbox{gray!30}{$B$. Effect of Source Query Set}} \\
        \midrule
        <NQ, MM> & 20.0 & 56.0 & 33.7 & 66.7 & 17.9 & 55.1 & 20.0 & 44.8 & \textbf{72.0} & \textbf{96.7} & 11.3 & 73.7 & 29.2 & 65.5 \\
        <MM, MM> & \textbf{23.7} & \textbf{61.3} & \textbf{47.1} & \textbf{76.7} & \textbf{33.5} & \textbf{68.7} & \textbf{30.1} & \textbf{51.8} & 70.0 & 69.9 & \textbf{20.1} & \textbf{83.3} & \textbf{37.4} & \textbf{68.6} \\
        \midrule
        <TQA, Wikipedia> & 23.1 & 61.0 & 43.9 & 77.3 & 18.4 & 54.6 & \textbf{23.9} & \textbf{47.6} & 62.5 & 92.9 & 15.4 & \textbf{79.2} & 31.2 & 68.8\\
        <SQA, Wikipedia> & 22.3 & 59.9 & \textbf{44.1} & \textbf{77.7} & 19.9 & 54.8 & 20.1 & 41.4 & 66.2 & 94.7 & \textbf{15.8} & 78.9 & \textbf{31.4} & 67.9\\
        <HQA, Wikipedia> & 18.4 & 54.6 & 34.6 & 69.7 & 11.4 & 37.4 & 18.3 & 40.6 & 46.5 & 83.8 & 10.5 & 69.1 & 23.3 & 59.2 \\
        <NQ$_\text{MRQA}$, Wikipedia> & \textbf{24.0} & \textbf{62.7} & 29.8 & 72.7 & \textbf{24.1} & \textbf{60.5} & \textbf{23.9} & 44.4 & \textbf{71.7} & \textbf{96.8} & 14.5 & 78.2 & 31.2 & \textbf{69.2}\\
        \hline\midrule
        \multicolumn{3}{l}{\colorbox{gray!30}{$C$. Effect of Source Document Set}} \\
        \midrule
        <NQ, Wikipedia> & \textbf{23.5} & \textbf{60.5} & \textbf{41.2} & \textbf{72.3} & \textbf{24.5} & \textbf{60.3} & \textbf{23.5} & \textbf{49.4} & \textbf{76.1} & \textbf{97.6} & 9.7 & 66.2 & \textbf{33.1} & \textbf{67.7}\\
        <NQ, MM> & 20.0 & 56.0 & 33.7 & 66.7 & 17.9 & 55.1 & 20.0 & 44.8 & 72.0 & 96.7 & \textbf{11.3} & \textbf{73.7} & 29.2 & 65.5\\
        <NQ, Wikipedia+MM> & 22.0 & 58.2 & 37.6 & 70.0 & 21.0 & 56.6 & 21.7 & 45.2 & 73.8 & 96.8 & 7.8 & 58.1 & 30.7 & 64.2 \\
        \hline\midrule
        \multicolumn{3}{l}{\colorbox{gray!30}{$D1$. Effect of Query Scale}} \\
        \midrule
        <NQ 10\%, Wikipedia> & 7.6 & 40.9 & 32.1 & 65.7 & 6.8 & 26.1 & 9.6 & 28.0 & 50.3 & 84.2 & 9.1 & 56.8 & 19.4 & 50.3\\
        <NQ 50\%, Wikipedia> & 22.1 & 59.6 & \textbf{38.7} & 70.0 & 18.9 & 54.8 & 18.0 & 42.4 & 61.4 & 92.4 & \textbf{12.0} & \textbf{71.9} & 28.5 & \textbf{65.2} \\
        <NQ 100\%, Wikipedia> & \textbf{23.0} & \textbf{59.7} & 36.8 & \textbf{71.3} & \textbf{20.6} & \textbf{55.9} & \textbf{18.9} & \textbf{44.4} & \textbf{65.8} & \textbf{94.0} & 10.1 & 65.2 & \textbf{29.2} & 65.1 \\
        \midrule
        <MM 10\%, MM> & 23.0 & 60.2 & 43.1 & 73.7 & 30.7 & 67.8 & 27.8 & 50.8 & 79.4 & 98.6 & 19.0 & 83.1 & 37.2 & 72.4\\
        <MM 50\%, MM> & \textbf{24.4} & 62.8 & 47.0 & 74.7 & 32.9 & 68.8 & 28.9 & 53.6 & 77.7 & 98.6 & 19.8 & 84.9 & 38.5 & 73.9 \\
        <MM 100\%, MM> & 23.4 & \textbf{62.9} & \textbf{47.6} & \textbf{77.7} & \textbf{34.0} & \textbf{69.4} & \textbf{31.8} & \textbf{55.6} & \textbf{80.1} & \textbf{99.0} & \textbf{20.7} & \textbf{85.4} & \textbf{39.6} & \textbf{75.0}\\
        \hline\midrule
        \multicolumn{3}{l}{\colorbox{gray!30}{$D2$. Effect of Document Scale}} \\
        \midrule
        <MMv2 1\%, MMv2> & \textbf{25.6} & \textbf{64.4} & 49.2 & \textbf{79.3} & 31.9 & 69.0 & \textbf{31.9} & \textbf{55.4} & \textbf{80.6} & \textbf{98.9} & \textbf{15.2} & \textbf{76.3} & \textbf{39.1} & \textbf{73.9} \\
        <MMv2 10\%, MMv2> & 24.7 & 63.6 & 48.2 & 78.0 & 32.1 & 66.7 & 30.2 & 54.6 & 77.9 & 98.7 & 14.4 & 75.1 & 37.9 & 72.8 \\
        <MMv2 100\%, MMv2> & 24.2 & 63.2 & \textbf{49.5} & \textbf{79.3} & \textbf{32.8} & \textbf{69.3} & 30.1 & 52.8 & 77.1 & 98.6 & 14.9 & 75.8 & 38.1 & 73.2\\
        \bottomrule
    \end{tabular}
    \caption{Zero-shot evaluation results on six target datasets. We use the form \emph{<Query Set, Document Set>} to denote the query and document sets used for training. }
    \label{tab:target-transfer}
    % In this paper, TQA, SQA, HQA, NQ, MM and MMv2 are the abbreviations for  TriviaQA, SearchQA, HotpotQA, Natural Questions, MSMARCO and MSMARCOv2, respectively.
\end{table*}



\subsection{The Effect of Source Query Set}
\label{sec:query-effect}
We first analyze the effect of different source query sets by fixing the document set. The examined query sets include NQ, MSMARCO, and datasets in MRQA~\cite{mrqa}. 

\subsubsection{Experimental Results}
\label{sec:query-exp}

First, we fix MSMARCO as the document set and use NQ queries and MSMARCO queries as two query sets to construct training data. 
% {Since MSMARCO queries only correspond to relevant document IDs in relevance judgments, we cannot construct training data using MSMARCO queries with Wikipedia~(initial document set of NQ)}. 
After training the backbone models with the two constructed training datasets~(denoted by $M_\text{NQ}$ and $M_\text{MARCO}$), we evaluate them on six target datasets.
Moreover, we collect four QA datasets in MRQA task as source datasets from similar domains, including TriviaQA, SearchQA, HotpotQA, and NQ.
Since these datasets are constructed based on Wikipedia, we adopt Wikipedia as the document set to construct training data for queries. By fixing the document set, we can analyze the effect of query sets on the retrieval performance. 


Table~\ref{tab:target-transfer}~(part $B$) shows the zero-shot retrieval results on six target datasets.  
It can be observed that the overall zero-shot capability on target datasets of $M_\text{NQ}$ is worse than $M_\text{MARCO}$, which is consistent with initial experiments (Table~\ref{tab:target-transfer}, part $A$). These results further verify that the source query set actually has important effects on the zero-shot capability of the DR model.
We also find that the model trained on HotpotQA shows the worst performance on target datasets. 
The reason may be that queries (primarily multi-hop questions) in HotpotQA are more challenging to answer, showing that special query formats may affect the zero-shot performance.
% It is because that  queries (primarily multi-hop questions) in HotpotQA are more challenging to answer, showing that query difficulty is a key factor in affecting the zero-shot performance.

Given the above overall analysis, we next zoom into two more detailed factors for better understanding the effect of the query set. 


\begin{figure}[!tb]
    \centering
    \subfigure[SciDocs]{\label{fig:overlap-scidocs}
		\centering
		\includegraphics[width=0.225\textwidth]{Img/overlap_scidocs.pdf}
	}
	\subfigure[SciFact]{\label{fig:overlap-scifact}
		\centering
		\includegraphics[width=0.225\textwidth]{Img/overlap_scifact.pdf}
	}
	\subfigure[FiQA]{\label{fig:overlap-fiqa}
 		\centering
		\includegraphics[width=0.225\textwidth]{Img/overlap_fiqa.pdf}
	}
	\subfigure[BioASQ]{\label{fig:overlap-bioasq}
		\centering
		\includegraphics[width=0.225\textwidth]{Img/overlap_bioasq.pdf}
	}
	\subfigure[Quora]{\label{fig:overlap-quora}
		\centering
		\includegraphics[width=0.225\textwidth]{Img/overlap_quora.pdf}
	}
	\subfigure[Arguana]{\label{fig:overlap-arguana}
		\centering
		\includegraphics[width=0.225\textwidth]{Img/overlap_arguana.pdf}
	}
    \caption{Relationship between vocabulary overlap and zero-shot performance on six target datasets. The $x$-axis corresponds to the sorted zero-shot performance on the target dataset of models trained on different source datasets. $y$-axis denotes the query/document overlap of source datasets and the target dataset.
    }
    \label{fig:overlap}
\end{figure}
\subsubsection{Query Vocabulary Overlap}
\label{sec:query-overlap}

 
Since domain similarity plays a key factor in cross-domain task performance~\cite{van2010using}, we first consider studying a simple yet important indicator to reflect the domain similarity, \ie the  vocabulary overlap between source and target query sets. We investigate how the vocabulary overlap of queries affects the zero-shot retrieval performance. 
Following the previous work~\cite{gururangan2020don}, we consider the top $10K$ most frequent words~(excluding stopwords) in each query set. For each pair of source query set and target query set, we calculate the percentage of vocabulary overlap by the weighted Jaccard~\cite{ioffe2010improved}.

Figure~\ref{fig:overlap}~(\emph{red lines}) present the relationship between query vocabulary overlap and zero-shot performance on six target datasets, where we sort the source datasets according to their corresponding results from Table~\ref{tab:target-transfer} ($x$-axis). The query vocabulary overlap between source and target datasets are shown in $y$-axis.


Overall, we can observe that \textbf{there is a certain positive correlation between query vocabulary overlap and zero-shot performance}, with only a small number of inconsistent cases. 
It is because a larger vocabulary overlap indicates a stronger domain similarity. 
Similar results~(\emph{blue lines} in Figure~\ref{fig:overlap}) are also found for vocabulary overlap of documents across domains.  


\begin{figure}[t]
    \centering
    \includegraphics[width=0.493\textwidth]{Img/query_type.pdf}
    \caption{Query type distribution on 11 datasets for each dataset with information entropy in last column, where top five datasets are source datasets and bottom six datasets are target datasets.}
    \label{fig:query_type}
\end{figure}

\subsubsection{Query Type Distribution}
\label{sec:query-type}
Besides vocabulary overlap, we continue to study the effect of another important factor, \ie query type distribution, which summarizes the overall distribution of query contents. In particular, we analyze the distribution of query types for both source and target query sets, focusing on ``WH'' queries, ``Y/N'' queries, and declarative queries. 
The query type is determined according to pre-defined rules, which are detailed in Appendix~\ref{app:query-rules}.


Figure~\ref{fig:query_type} presents the distribution of each query set from 11 source and target datasets. For better understanding such a distribution, we also calculate the information entropy~\cite{shannon1948mathematical} of query type distribution for each dataset, where a larger entropy value indicates a more balanced distribution of query types. First, we find that
%The larger the value is, we consider that a larger value indicates a more diverse distribution of query types on that dataset. First, we speculate that
\textbf{models trained with more comprehensive query types are capable of performing better in the zero-shot retrieval setting}, \eg MSMARCO dataset. In particular, MSMARCO contains the most diverse and comprehensive queries among all source datasets, which leads to a more strong zero-shot capability of DR models as the source training set.   

Furthermore, \textbf{when source and target query sets share more similar query type distributions, the corresponding zero-shot performance is also likely to improve}.
For example, SearchQA, containing a large proportion of declarative queries, performs better on datasets also with a large proportion of declarative queries, such as ArguAna and SciFact. 



\subsection{The Effect of Source Document Set}
\label{sec:document-effect}
Following the analysis of query sets, we next study the effect of source document sets. 

To conduct the analysis, we fix NQ queries as the source query set and use Wikipedia and MSMARCO as source document sets. 
Furthermore, we merge the Wikipedia and MSMARCO document sets as a more comprehensive document set to study the effect of additional documents from other domain. For each query, we can use the short answer annotated in NQ dataset to select documents from three document sets to construct training data. 
After training with different source datasets (same query set but different document sets: Wikipedia, MSMARCO, and their combination), we evaluate the zero-shot performance of these three models on six target datasets.

Table~\ref{tab:target-transfer}~(part $C$) provides the evaluation results  on six target datasets. A surprising finding is that \textbf{the model trained on the merged document set does not outperform the model trained on Wikipedia on target datasets}. 
A possible reason is that short answers of NQ queries annotated based on Wikipedia do not match well for other document sets, resulting in performance degradation. On the whole, the effect of the underlying document set is not that significant as query set. 


\subsection{The Effect of Data Scale}
\label{sec:data-scale}
Since DR models highly rely on training data, it is also important to consider the effect of data scale of source training set. 

\begin{table}[t]
    \scriptsize
    \centering
    % \renewcommand\tabcolsep{4.3pt}
    \begin{tabular}{l|c|cc}
        \toprule
        \textbf{Target~($\rightarrow$)} & \textbf{Query} & \multicolumn{2}{c}{\textbf{In-domain}}\\
        \textbf{Source~($\downarrow$)} & \textbf{Scale} & \textbf{M@10} & \textbf{R@50}   \\
        \midrule
        <NQ 10\%, Wikipedia> &5K & 40.2 & 76.1   \\
        <NQ 50\%, Wikipedia> & 25K & 53.4 & 84.1  \\
        <NQ 100\%, Wikipedia> & 50K & \textbf{56.8} & \textbf{85.0}   \\
        \midrule
        <MM 10\%, MM> & 50K  & 30.8 & 79.5  \\
        <MM 50\%, MM> & 250K  & 33.8 & 83.0  \\
        <MM 100\%, MM> & 500K  & \textbf{34.9} & \textbf{83.5} \\
        \bottomrule
    \end{tabular}
    \caption{In-domain experiments on NQ and MSMARCO by varying  different ratios of  queries from the original query set.}
    \label{tab:query-scale}
\end{table} 

\subsubsection{Query Scale}
\label{sec:query-scale}
Query scale refers to the number of queries in the source training set. Since each training query corresponds to one (or multiple) labeled document(s) for retrieval tasks, query scale represents the amount of annotated data. We conduct experiments on NQ and MSMARCO by varying the query scale. For each dataset, we randomly sample 10\%, 50\%, and 100\% queries from the training set and construct three training sets. We use these training sets of different proportions to train the models separately and conduct in-domain and out-of-domain evaluations.

Table~\ref{tab:query-scale} presents the results of in-domain evaluation and Table~\ref{tab:target-transfer}~(part $D1$) presents the out-of-domain results on six target datasets.
First, \textbf{with the increase of the query scale in the training set, the in-domain capability and out-of-domain zero-shot capability of models gradually improve}.
% Although zero-shot performance and query scale seem to be positively correlated, it is more sensitive to query scale when training data achieves. 
Furthermore, considering the two settings with the same query scale, \ie ``NQ 100\%'' and ``MSMARCO 10\%'' with 50K queries, we find the model trained on  ``MSMARCO 10\%'' still achieves a better zero-shot performance than that trained on ``NQ 100\%''. 
Combining the results in Section~\ref{sec:initial-analysis}, we find the stronger zero-shot capability of model trained on MSMARCO dataset does not simply come from the larger query scale. 

\begin{table}[t]
    \scriptsize
    \centering
    \renewcommand\tabcolsep{2.2pt}
    \begin{tabular}{l|cc|cc|cc}
        \toprule
        \textbf{Target~($\rightarrow$)} & \multicolumn{2}{c|}{\textbf{MMv2 100\%}} & \multicolumn{2}{c|}{\textbf{MMv2 10\%}} & \multicolumn{2}{c}{\textbf{MMv2 1\%}} \\
        \textbf{Source~($\downarrow$)} & \textbf{M@10} & \textbf{R@50} & \textbf{M@10} & \textbf{R@50} & \textbf{M@10} & \textbf{R@50}  \\
        \midrule
        BM25 & 6.4 & 24.7 & 16.7 & 44.8 & 31.3 & 63.6 \\
        <MMv2, MMv2 100\%> & \textbf{20.6} & \textbf{63.7}  & \textbf{44.0} & \textbf{86.2}  & 61.7 & 93.7 \\
        <MMv2, MMv2 10\%> & {20.4} & {63.3} & \textbf{44.0} & {86.0}  & {62.0} & {94.0} \\
        <MMv2, MMv2 1\%> & 16.4 & 59.1 & 40.0 & 84.8 & \textbf{62.3} & \textbf{94.5}\\
        \bottomrule
    \end{tabular}
    \caption{Experiments with varying document scales on MSMARCOv2.}
    \label{tab:corpus-scale}
\end{table}

\subsubsection{Document Scale}
\label{sec:document-scale}
We further analyze the effect of document scale using MSMARCOv2~(passage) dataset~\cite{msmarcov2}, which is the largest publicly available text collection up to date.  

Concretely, we randomly sample two subsets of 1\% (1.4 million) and 10\% (14 million) from MSMARCOv2 document set. 
In each setting, we fix the training queries and corresponding annotations, while the negatives for training are specially constructed from different document sets.
We train three different models with 1\%, 10\%, and full document sets, and apply each model on MSMARCOv2 development set for examining the results with different document scales.
More details can be found in Appendix~\ref{app:document-scale}.


\paratitle{In-domain Evaluation} Table~\ref{tab:corpus-scale} presents the zero-shot retrieval results with different document scales in the source training data. It seems that the model trained on a larger document set shows better retrieval capacity for in-domain evaluation. 
Moreover, we find that the performance decrease of DR model is not as significant as that of BM25 when increasing the document scale for evaluation, which is different from the findings of previous work~\cite{reimers2020curse}. A possible reason is that they utilize synthetic data to construct large document set, which have a large gap with the actual scene, and cannot be well addressed by DR model.


\paratitle{Out-of-domain Evaluation} We also evaluate the models trained with different document scales on six target datasets and report the results in  Table~\ref{tab:target-transfer}~(part $D2$). 
Surprisingly, the model trained on 1\% document set outperforms those trained on the full document set and 10\% document set, which seems to contradict the intuition. 
We suspect that since the discrepancies of training sets are negatives, the DR model is trained with more diverse source domain negatives using a larger document set, which absorbs more domain-specific characteristics. Therefore, the trained DR model with a larger document set is likely to lead to over-fitting issue in cross-domain setting.
Overall, \textbf{it is useful to increase the scale of the document set for improving in-domain performance, but may hurt out-of-domain performance}.



\begin{figure}[t]
    \centering
    \includegraphics[width=0.38\textwidth]{Img/bias.pdf}
    \caption{Relationship between the improvement ratio of DR models over BM25 and the the overlap coefficient of different target datasets.}
    \label{fig:bias}
\end{figure}

\subsection{The Bias from Target Datasets}
\label{sec:bias}

% In previous experiments, we mainly examine the effect of source training data. Here, we incorporate target data (test set) for further analysis.
Recently, BEIR~\cite{thakur2021beir} points out that sparse models are often used to create the annotation data for dataset construction, resulting in the lexical bias on target datasets.
According to this, we consider quantitatively investigating how such bias affects the zero-shot performance of the sparse and dense retrieval models, by computing the overlap coefficient~\cite{vijaymeena2016survey} over queries and annotated documents in target test sets.
% Here, we compute the term overlap over queries and annotated documents in test sets, and examine how this overlap ratio affects the zero-shot performance of sparse and dense retrieval models. 

Specially, for each query from the test set of the target dataset, we compute the overlap coefficient by dividing the number of the overlap terms of the query and the annotated document by the total number of query terms. We compute the overlap coefficient for six target datasets, and sort them according to the value ascendingly. In particular, we mainly consider comparing sparse and dense retrieval models.
The results of different overlap coefficient for the six target datasets are shown in Figure~\ref{fig:bias}. It can be observed that \textbf{BM25 overall performs better on the target dataset with a larger overlap coefficient and the performance of DR models is better than BM25 with a low overlap coefficient}. 
This finding indicates that the bias of the target dataset may cause it to fail to evaluate the zero-shot capabilities of different models accurately. Thus, how to construct fair datasets is also an important direction that needs to be further explored.
%using sparse retrieval models for dataset constructing may bring high overlap coefficient between queries and annotated documents, resulting in the natural advantage for BM25.
An exception in Figure~\ref{fig:bias} is the Quora dataset. It is because that this dataset is created for duplicate question identification, where the query and the document annotation are two related questions with a larger surface similarity.

% Indeed, when the query term overlapping proportion is high, it is potentially more favorable for sparse retrieval models that rely on exact match. This indicates that there might exist performance comparison bias in existing benchmarks. Such a bias has also been noted in the BEIR~\cite{thakur2021beir}, where sparse models are often used to create the annotation data for dataset construction. 


\subsection{Summarizing the Main Findings}
In this part, we summarize the main findings based on the above experimental analysis.

First, source training set has important effect on the zero-shot retrieval capacities~(Section~\ref{sec:query-effect} and~\ref{sec:document-effect}), since DR models need to be trained on it. 
Various factors related to source training set will potentially affect the zero-shot performance, including vocabulary overlap~(Section~\ref{sec:query-overlap}) and query type distribution~(Section~\ref{sec:query-type}).
Our empirical study shows that it is useful to improve the zero-shot performance by increasing the vocabulary overlap and query type distribution similarity between source and target domains and setting more balanced query type distributions for the source domain.


Second, query scale of source training data significantly affects the zero-shot capability, and increasing the query scale (the amount of annotation data) brings performance improvement on both in-domain and out-of-domain performance~(Section~\ref{sec:query-scale}). However, it seems to bring negative effect when increasing the document scale, which shows a performance decrease in our experiments~(Section~\ref{sec:document-scale}). 

Third, when the test set has a large overlap coefficient between queries and annotated documents, the evaluation might be biased towards exact matching methods such as BM25~(Section~\ref{sec:bias}). 

Finally,  we find that MSMARCO seems to be a more capable source dataset for training zero-shot DR models, compared with NQ. The major reason is that it contains more queries, covers more comprehensive terminologies that may appear in other domains, and has a more balanced distribution of query types.


==> Zero-shot Dense Retrieval/subfile/4_method.tex <==
\section{Model Analysis}
So far, we mainly focus on the discussions of data side. In this section, we further review and analyze existing zero-shot DR models.  

\subsection{Reviewing Existing Solutions}
\label{sec:organization}
According to the specific implementations, we summarize the existing 
zero-shot DR models with the adopted techniques in Table~\ref{tab:methods}. Next, we discuss the major techniques and the representative methods. Note that this section is not a comprehensive list of existing studies, but rather an analysis of the different techniques they use and factors from the previous analysis they improve on.

\begin{table}[]
\scriptsize
\centering
\begin{tabular}{c|ccccc|c}
    \toprule
    \textbf{Method} & \textbf{QG} & \textbf{KD} & \textbf{CP} & \textbf{MSS} & \textbf{ISR} & \textbf{Factors} \\
    \midrule
    QGen &  \checkmark &  &  &  && VO+QT+QS\\
    % \cline
    % AugDPR & \checkmark &  &  &  && VO+QT+QS\\
    % \cline
    AugSBERT &  & \checkmark &  & && QS \\
    % \cline
    SPAR &  & \checkmark  & &  & \checkmark & QS \\
    GPL & \checkmark & \checkmark &  & &&  VO+QT+QS\\
    % \cline
    Contriever & & & \checkmark&& & QS\\
    % \cline
    GTR &  &  &&  \checkmark & &QS  \\
    % \cline
    % RRF &  &  &  & \checkmark & & VO\\
    LaPraDoR & & & \checkmark& & \checkmark  & QS\\    
    \bottomrule
\end{tabular}
\caption{Representative zero-shot DR methods with different techniques. We mark the corresponding influence factors of each methods, where VO, QT, and QS denote the improving factors of vocabulary overlap, query type and query scale, respectively.}
\label{tab:methods}
\end{table}

\paratitle{Query Generation~(QG)} 
QG methods construct synthetic training data by using documents from the target domain to generate corresponding (pseudo) queries, which aims to augment the training data by generating queries that fit the target domain.
QGen~\cite{ma2021zero} trains an Auto-encoder in the source domain to generate synthetic questions by a target domain document.
Similarly, GPL~\cite{wang2021gpl} generates synthetic queries with a pre-trained T5 model.
QG can enhance the vocabulary overlap between the source and target domains, meanwhile increasing the query scale and fitting the query type distribution of the target domain. 


\paratitle{Knowledge Distillation~(KD)}
KD is a commonly used strategy in DR, which utilizes a powerful model~(\eg cross-encoder) as the teacher model to improve the capabilities of DR models~\cite{tasbalanced2021, pair}. It has been found that such a technique can improve out-of-domain performance~\cite{thakur2020augmented}.
GPL~\cite{wang2021gpl} and AugSBERT~\cite{thakur2020augmented} use cross-encoder to annotate unlabeled synthetic query-doc pairs to train the bi-encoder. Different from the above methods, SPAR~\cite{chen2021salient} proposes to distill knowledge from BM25 to DR model.
KD based approaches alleviate the data scarcity issue and play a similar role in increasing the query scale (\ie more supervision signals). 

\paratitle{Contrastive Pre-training~(CP)} With unsupervised contrastive learning showing great power in the field of NLP, researchers start to apply this approach to zero-shot DR. 
Contriever~\cite{izacard2021towards} and LaPraDoR~\cite{xu2022laprador} are two typical methods that build large-scale training pairs similar to SimCSE~\cite{gao2021simcse} and utilize contrastive loss in training.
Such approaches use unsupervised corpus to construct training data, allowing the model to capture the matching relationship between two text contents in the pre-training phase, essentially enlarging the training data scale.

\paratitle{Model Size Scaling~(MSS)} For PLM based approaches, it becomes a broad consensus that scaling the model size can lead to substantial performance improvement~\cite{brown2020language, fedus2021switch}. 
%Model size is one of the characteristics of the model itself, independent of the data perspective. Thereby scaling the model size is a pure methodological improvement. It has become a broad consensus in natural language processing that scaling the model size can improve performance consistently. 
Recently, MSS has shown the effectiveness in zero-shot DR. GTR~\cite{Ni2021LargeDE} is a generalizable T5-based DR model that uses extremely large-scale training data and model parameters, which obtain performance gains.
% is pre-trained on 2 billion generic question-answer pairs and has up to 5 billion parameters for better generalization ability on out-of-domain datasets, which shows the performance gains from extremely large model and training data. 


\paratitle{Integrating Sparse Retrieval~(ISR)} 
It has been shown that both sparse and dense retrieval models have specific merits when dealing with different datasets. Thus, it is an important practical approach that integrates the two kinds of methods for enhancing the zero-shot retrieval capacities. 
SPAR~\cite{chen2021salient} utilizes a student DR model that distills BM25 to the DR model, then concat the embeddings from the BM25-based DR model and a normal DR model. Moreover, LaPraDoR~\cite{xu2022laprador} enhances the DR model with BM25 by multiplying the BM25 score with the similarity score of DR model.
We consider ISR as a special approach because it does not change the setup of source training set for DR model, but mainly combines the sparse and dense models in an ensemble way.



\begin{table}[t]
\scriptsize
\centering
\begin{tabular}{llccc}
\toprule
\textbf{Method} & \textbf{PLM} & \textbf{BioASQ} & \textbf{SciFact} & \textbf{FiQA} \\
\midrule
BM25 & \textbf{-} & {46.5} & 66.5 & 23.6 \\
\midrule
QGen & DistilBERT & 39.8 & 64.4 & 30.8 \\
% Contriever & BERT$_\text{base}$ & - & \underline{67.7} & 32.9 \\
GTR & T5$_\text{base}$ & 27.1 & 60.0 & \textbf{34.9} \\
GPL & DistilBERT & \underline{42.5} & \underline{65.2} & \underline{33.1} \\
LaPraDoR & DistilBERT & \textbf{51.1} & \textbf{68.7} & 34.3 \\
LaPraDoR$_\text{w/o LEDR}$ & DistilBERT & 30.8 & 59.9 & 31.4 \\
\bottomrule
\end{tabular}
\caption{NDCG@10 results of different zero-shot methods on three target datasets. }
\label{tab:performance}
\end{table}

\subsection{Comparison of Zero-shot Methods}
We compare different zero-shot methods on the three most commonly used target datasets for existing zero-shot methods, including BioASQ, SciFact, and FiQA. Concretely, we show the results of QGen reported in BEIR since the results in QGen paper is incomplete, and we report the T5$_\text{base}$ results in GTR paper for fair comparison.  We replicate the results of GPL on BioASQ with the full document set, since the results in GPL paper is performed by randomly removing irrelevant documents in the document set. For LaPraDoR, we use the results of ``FT'' version that the model is finetuned on MSMARCO dataset. We also report the results that implement without considering BM25 scores~(w/o LEDR) for LaPraDoR to investigate the effect of incorporating BM25.
Table~\ref{tab:performance} reports the performance comparison of these zero-shot methods.

First, we can see that LaPraDoR overall outperforms other DR models, when remove the BM25 enhanced strategy, there is a huge drop in the zero-shot performance on BioASQ and SciFact. This corresponds to our previous analysis~(Section~\ref{sec:bias}), introducing BM25 in DR model can greatly improve the zero-shot performance on datasets with high overlap proportion (BioASQ and SciFact), while it does not bring much performance improvement on FiQA that has low overlap proportion.
Without considering ISR, GPL achieves competitive performance, since it mainly fits for the vocabulary overlap and query type between the source and target domains, as well as increases the scale of pseudo labeled data (for training with knowledge distillation). 
Considering more positive influence factors does bring the DR model a zero-shot performance improvement.
% In addition, we also find that existing methods (except ISR method) are still worse than BM25 on BioASQ and SciFact, since these two datasets are created by relying on heavily on term matching.
 %As one of our conclusions, such datasets in the presence of bias rely heavily on terminology matching. Therefore, the zero-shot capability of the DR model still needs to be further improved.

\ignore{
\begin{table}[]
    \centering
    \scriptsize
    \begin{tabular}{l|l|c|c}
        \toprule
        \textbf{Target Dataset} & \textbf{Type} & \textbf{RetM} & \textbf{RetR} \\
        \midrule
        \multirow{2}{*}{MSMARCO} & zero-shot evaluation & 21.0 & 64.5 \\
         & zero-shot learning & \textbf{26.6} & \textbf{69.1} \\
         \midrule
        \multirow{2}{*}{FiQA-2018} & zero-shot evaluation & 23.9 & 61.6 \\
         & zero-shot learning & \textbf{27.3} & \textbf{64.0} \\
        \midrule
        \multirow{2}{*}{SciFact} & zero-shot evaluation & 40.5 & 73.7 \\
         & zero-shot learning & \textbf{48.3} & \textbf{79.7} \\
         \bottomrule
    \end{tabular}
    \caption{The comparison of zero-shot evaluation and distillation-based zero-shot learning, which using NQ as the source dataset.
    }
    \label{tab:distillation}
\end{table}

\subsection{Distillation-based Zero-shot Transfer}
Based the empirical analysis on the four influencing factors, we find that increasing the query scale and fitting the query and document distribution on the source and target domain are beneficial to enhance the transfer capability of models. In addition, the zero-shot capability of re-ranker is generally stronger than that of retriever. Therefore, considering these conclusions, we propose to use the re-ranker as teacher (re-ranker zero-shot capability is strong), leverage large-scale unsupervised queries (increase query scale) and corpus on target domain (fitting query corpus distribution), and distill the knowledge from teacher to retriever.

Concretely, based on the advantages of the joint training system of retriever and re-ranker, we naturally have a well-trained re-ranker. Therefore, similar to previous works~\cite{pair, thakur2020augmented}, our idea is distill the knowledge of re-ranker to retriever. We use the retriever trained in the source domain to retrieve top-$k$ instances on the target corpus using existing unsupervised target domain queries. After that, we use the re-ranker to provide relevance scores of the recall results, and set two thresholds according to the characteristics of the target field to filter positive and negative distilled instances as training data. We conduct the experiment using NQ as the source dataset and choose MSMARCO, FiQA-2018 and SciFact as target datasets for evaluation. 

As seen in Table~\ref{tab:distillation}, the proposed distillation-based zero-shot strategy shows extraordinary performance comparing to zero-shot evaluation on the three datasets. Additionally, we observed that the performance of model trained on FiQA-2018 virtually rivals the performance of BM25. As mentioned before, BM25 has advantages on target datasets with relatively specific domains due to its lexical matching ability. Therefore, it shows that although the zero-shot capability of DR model is not strong enough on specific domain, its transfer capability can be greatly improved through a unsupervised data on target domain.


\begin{figure}
	\centering
	\includegraphics[width=0.43\textwidth]{Img/few-shot.pdf}
	\caption{Results of few-shot learning on MSMARCO.}
	\label{fig:few-shot}
\end{figure}

\subsection{Few-shot Transfer}
Another common transfer scenario is that a small amount of target domain annotated data is avaliable, \ie few-shot scenario. Therefore, we first randomly sample subsets of different scales from queries in MSMARCO training set, construct training data based on MSMARCO corpus, and re-train the model trained on NQ to evaluate the model performance under different data scales.

Figure~\ref{fig:few-shot} presents the evaluation results on MSMARCO. As we can see, using 1\% of the data can achieve 50\% improvement in the performance of using the full amount of data. Continue to increase the amount of data, the increase speed is significantly slowed. The performance improvement in the last 50\% of the training data is only about 1\%. This observation supplements the previous conclusion that training on a small amount of supervised data on target domain can also improve the transfer capability of DR model.


In addition, we attempt to borrow the idea from active learning~\cite{settles2009active} to improve few-shot learning by filtering the few-shot data. Interestingly, we observe that the few-shot performance of active learning method did not surpass the original randomly sampled training data. Detail description can be found in Appendix~\ref{app:active-learning}.
}






==> Zero-shot Dense Retrieval/subfile/5_related.tex <==
\section{Related Work}
% \subsection{Dense Retrieval and Re-ranking}
\paratitle{Dense Retrieval} 
In recent years, dense retrieval has been proved that outperforms traditional term-based approaches~(\eg TF-IDF and BM25) on a number of scenarios. One line of dense retrieval studies is pre-training for dense retrieval~\cite{gao2021unsupervised, ouguz2021domain, REALM, latent2019acl}, which usually incorporates task-specific loss during pre-training process~\cite{pair, gao2021condenser, pretrain2020iclr}. While another line is fine-tuning pre-trained language models with supervision, where a number of studies attempt to figure out challenges in dense retrieval, \eg negative sampling~\cite{Optimizing2021sigir, ANCE, rocketqa}, improving efficiency~\cite{zhan2021jointly}, and conduct end-to-end training~\cite{sachan2021end, rocketqav2}.
% Re-ranking is a follow-up stage of first-stage retrieval. Recently, PLM-based re-rankers have been widely applied~\cite{qiao2019understanding, nogueira2019passage, Gao2020ModularizedTR} and yield substantial improvements over the traditional methods~\cite{jegou2011searching} based on rich contextualized matching mechanisms.
% Considering the dependency and relevance between dense retrieval and re-ranking, RocketQAv2~\cite{rocketqav2} proposes a joint training system of retriever and re-ranker. Since RocketQAv2 achieves extraordinary performance and has simple process to simultaneously train a retriever and a re-ranker, we adopt it to conduct the analytical experiments.

\paratitle{Zero-shot Dense Retrieval}
Nowadays, as dense retrieval has received great attention, several studies have begun to focus on the zero-shot capabilities of dense retrievers. Due to the lack of  large-scale in-domain training data for retrieval task, the zero-shot capability of the dense retrieval model largely determines its robustness and generality.
BEIR~\cite{thakur2021beir} proposes a heterogeneous evaluation benchmark for information retrieval and points out the weakness of dense retrieval on zero-shot evaluation. In addition, there is a series of works looking at ways to improve zero-shot performance, which is described in detail in Sec.~\ref{sec:organization}.
Different from previous works, we provide a comprehensive and in-depth analysis of the zero-shot capability of dense retrieval and examine how influencing factors affect such capability.

==> Zero-shot Dense Retrieval/subfile/6_conclusion.tex <==
\section{Conclusion and Future Work}

In this paper, we thoroughly examine the zero-shot capability of DR models. We conduct empirical analysis by extensively studying the effect of various factors on the retrieval performance. 
In particular, we find that the factors of vocabulary overlap, query type distribution, and data scale are likely to affect the zero-shot performance of dense retriever.
Besides, the performance between BM25 and DR models varies significantly on different target datasets, where the dataset bias (\eg a dataset is created based on exact match) is likely to make such comparison unfair. 
Overall, we find that the zero-shot performance of dense retrieval models still has room to improve and deserves further study.

As future work, we will consider designing more robust, general zero-shot retrieval methods that can well adapt to different settings or domains. 

==> subfile/5_related.tex <==
\section{Related Work}
% \subsection{Dense Retrieval and Re-ranking}
\paratitle{Dense Retrieval} 
In recent years, dense retrieval has been proved that outperforms traditional term-based approaches~(\eg TF-IDF and BM25) on a number of scenarios. One line of dense retrieval studies is pre-training for dense retrieval~\cite{gao2021unsupervised, ouguz2021domain, REALM, latent2019acl}, which usually incorporates task-specific loss during pre-training process~\cite{pair, gao2021condenser, pretrain2020iclr}. While another line is fine-tuning pre-trained language models with supervision, where a number of studies attempt to figure out challenges in dense retrieval, \eg negative sampling~\cite{Optimizing2021sigir, ANCE, rocketqa}, improving efficiency~\cite{zhan2021jointly}, and conduct end-to-end training~\cite{sachan2021end, rocketqav2}.
% Re-ranking is a follow-up stage of first-stage retrieval. Recently, PLM-based re-rankers have been widely applied~\cite{qiao2019understanding, nogueira2019passage, Gao2020ModularizedTR} and yield substantial improvements over the traditional methods~\cite{jegou2011searching} based on rich contextualized matching mechanisms.
% Considering the dependency and relevance between dense retrieval and re-ranking, RocketQAv2~\cite{rocketqav2} proposes a joint training system of retriever and re-ranker. Since RocketQAv2 achieves extraordinary performance and has simple process to simultaneously train a retriever and a re-ranker, we adopt it to conduct the analytical experiments.

\paratitle{Zero-shot Dense Retrieval}
Nowadays, as dense retrieval has received great attention, several studies have begun to focus on the zero-shot capabilities of dense retrievers. Due to the lack of  large-scale in-domain training data for retrieval task, the zero-shot capability of the dense retrieval model largely determines its robustness and generality.
BEIR~\cite{thakur2021beir} proposes a heterogeneous evaluation benchmark for information retrieval and points out the weakness of dense retrieval on zero-shot evaluation. In addition, there is a series of works looking at ways to improve zero-shot performance, which is described in detail in Sec.~\ref{sec:organization}.
Different from previous works, we provide a comprehensive and in-depth analysis of the zero-shot capability of dense retrieval and examine how influencing factors affect such capability.
